Safe Control for Nonlinear Systems with Stochastic Uncertainty via Risk Control Barrier Functions

Guaranteeing safety for robotic and autonomous systems in real-world environments is a challenging task that requires the mitigation of stochastic uncertainties. Control barrier functions have, in recent years, been widely used for enforcing safety related set-theoretic properties, such as forward invariance and reachability, of nonlinear dynamical systems. In this paper, we extend this rich framework to nonlinear discrete-time systems subject to stochastic uncertainty and propose a framework for assuring risk-sensitive safety in terms of coherent risk measures. To this end, we introduce risk control barrier functions (RCBFs), which are compositions of barrier functions and dynamic, coherent risk measures. We show that the existence of such barrier functions implies invariance in a coherent risk sense. Furthermore, we formulate conditions based on finite-time RCBFs to guarantee finite-time reachability to a desired set in the coherent risk. Conditions for risk-sensitive safety and finite-time reachability of sets composed of Boolean compositions of multiple RCBF are also formulated. We show the efficacy of the proposed method through its application to a cart-pole system in a safety-critical scenario.

==> Figures/walkingExample.tex <==

In previous section, we used a numerical example to elucidate our proposed methodology. In the following, we demonstrate the application of risk barrier functions for bipedal walking. A linear discrete dynamics is used to approximate (with uncertainties) the actual step-to-step (S2S) dynamics of the robot walking for step planning. More details about the step planning can be found in \cite{xiong2021inReview}. Here we briefly describe the stepping controller, the problem setups, and the applications of risk barrier functions.
  
\subsubsection{Stepping Controller for Walking}
The walking of the robot is modeled as a hybrid dynamical system which is composed by continuous dynamics and discrete transitions \cite{grizzle2014models}. We use the general two-domain hybrid system of walking; the continuous dynamics is thus composed by a single support phase (SSP) and a double support phase, and the discrete transitions are between the SSP and DSP. We apply the Hybrid-Linear Inverted Pendulum (H-LIP) based approach in \cite{xiong} to synthesis and stabilize walking gait. The walking behavior, i.e., the horizontal center of mass (COM) trajectory, is controlled by the step size based on the step-to-step dynamics approximation via the H-LIP. The S2S dynamics of the robot is 
\begin{equation}
\label{eq:S2S}
    \mathbf{x}_{k+1} = A \mathbf{x}_k + B u_k +w 
\end{equation}
where $\mathbf{x}$ is the discrete horizontal COM state at the pre-impact event, $u$ is the step size on the robot, $A$ and $B$ are the matrices of the linear S2S dynamics of the H-LIP, and $w$ is the difference of the S2S dynamics between the robot and the H-LIP.  
The step size on the robot is calculated based on the H-LIP stepping:
\begin{equation}
    u = u^\text{H-LIP} + K (\mathbf{x} -\mathbf{x}^\text{H-LIP}  )
\end{equation}
which makes sure that the robot state is close to the state of the H-LIP $\mathbf{x}^\text{H-LIP}$; $K$ is a feedback gain to make $A+BK$ stable. In the later, we use the disturbed linear dynamics in Eq. \eqref{eq:S2S} to plan for walking behaviors on the H-LIP and then apply the H-LIP stepping to realize the walking on the robot. Barrier functions are synthesized for guaranteeing safety on the robot walking. 


\subsubsection{Problem Definition}
We consider the following scenarios of controlling the robot. 
  
\noindent{\textbf{Reaching a Target Region:}} We consider a case where the robot should walk to reach to a target square region, which is defined via four barrier functions. Without the barrier function, the robot is supposed to walking in place with not horizontal velocity. By integrating the barrier function in the planning via the H-LIP based controller, the robot walks to the target region and stays inside.

  
\noindent{\textbf{Path Tracking with Obstacle Avoidance:}} We also consider a case where the robot walks to follow a path with obstacles along the path. The barrier functions are designed to represent collision-free regions in the space. Here we demonstrate the walking without and with the barrier functions. Without the barrier functions in the controller, the robot precisely follows the path but then inevitably collides with the obstacles. With the barrier functions, the robot follows the path when it can and avoids obstacles when it has to.


==> Sections/experiments_old.tex <==
  \section{Experiments} \label{sec:experiments}
  
  In this section, we illustrate the proposed method by two examples, namely, a numerical example and a case study. The associated optimization problems are solved in CVX using MOSEK solver at each step. The computations were carried out on a laptop computer with the processor intel(R) Core(TM) i7-7700HQ @2.8GHz and 16GB of RAM.
  
  \subsection{Example I: Numerical Example}
  
      \begin{figure*}[!h] \centering{
%\includegraphics[scale=.3]{mdpexample.png}\\
\includegraphics[scale=.13]{Figures/Figmean.png}~
\hspace{1cm}
\includegraphics[scale=.13]{Figures/Figcvar.png}
\hspace{1cm}
\includegraphics[scale=.13]{Figures/Figevar.png}
\vspace{-0cm}
\caption{Risk-sensitive safety enforcement results for the Example I with total expectation (left), CVaR (middle), and EVaR (right) coherent risk measures for 50 Monte Carlo simulations. The red shaded area denotes the unsafe region.}\label{fig:mdp}
%\vspace{-0.5cm}
} 
 \end{figure*}
  
  Consider the following discrete-time system with stochastic uncertainty
  \begin{equation} \label{eq:dcpcvrrrar}
      x^{t+1}= \begin{bmatrix} 1 & 2+w^t \\ 2 & 2+w^t \end{bmatrix} x^t + \begin{bmatrix} 1 \\ 2 \end{bmatrix} u, \quad x_0 = \begin{bmatrix}-1\\ 1\end{bmatrix},
  \end{equation}
  where the uncertain parameter satisfies $w \in \{-0.5,0.5\}$ with $p(w=0.5)=0.5$ and $p(w=-0.5)=0.5$. 
  
  \subsubsection{$\rho$-safety} We are interested in enforcing risk-sensitive safety for the following safe set
  $$
 \mathcal{S} = \left \{ x \in \mathbb{R}^2 \mid \begin{bmatrix}1 & 0\end{bmatrix}x+2\ge 0 \right\}.
  $$
  Hence, by definition~\eqref{eq:safeset}, we have 
  $$
  h(x) = \begin{bmatrix}1 & 0\end{bmatrix}x+2.
  $$
  We consider three coherent risk measures, namely, conditional expectation, CVaR, and EVaR. As highlighted in Section~\ref{sec:DCPcomput}, in the conditional expectation case, CVaR case, and the EVaR case, we solve quadratic program~\eqref{eq:DCP} with~\eqref{cscseee}, DCP~\eqref{eq:dcpcvar}, and DCP~\eqref{eq:DCPevar}, respectively. The control bounds were chosen as $u \in [-5,5]$.
  
  Table I summarizes the results from numerical experiments. For each Monte Carlo simulation, we select the initial condition from a uniform random distribution in the safe set $\mathcal{S}$. For CVaR and EVaR measures, we designed the risk-sensitive safe controller for three different confidence levels of $\beta =0.1,0.5,08$ ranging from more to less risk-sensitive measures.  Average Time illustrates the average time spent at every time step solving the associated optimization to design the risk-sensitive safe controller. Failure ratio signifies the number of times the trajectories violated the safety constraint $h(x)\ge 0$ in the 100 Monte Carlo runs. 
  
  It can be inferred from Table I that, while in the case of conditional expectation computations are carried out relatively faster (solving a QP) than the risk-sensitive cases, the risk-neutral controller leads to a significantly higher number of safety violations due to stochastic uncertainty. On the other hand, the risk-sensitive cases of CVaR and EVaR incur more computations (solving DCPs) but lead to much less safety violations especially for higher values of $\beta$. Lastly, we note that EVaR-based controller fared better compared to CVaR-based one in terms of number of failures. Indeed, this is consistent with the theory that EVaR is a more conservative coherent risk measure than CVaR, i.e., $\mathbb{E}(h)\ge \mathrm{CVaR}_\beta(h) \ge \mathrm{EVaR}_\beta(h)$~\cite{ahmadi2012entropic}. 
  
  \begin{table}[t!]
\label{table:comparison}
\centering
\setlength\tabcolsep{2.5pt}
\begin{tabular}{lccccc} \midrule
\makecell{Risk Measure} & \makecell{$\beta$}  &  \makecell{ Average   Time [s] }  & \makecell{ Failure Ratio}   \\ 
\midrule $\mathbb{E}$ &
--            & 0.06                & 29\%                                        \\[1.5pt]
\midrule
$\mathrm{CVaR}$ & 0.8            & 0.12                                      &16\%                                            \\[1.5pt]
$\mathrm{CVaR}$ & 0.5           & 0.11                                    &11\%                                          \\[1.5pt]
$\mathrm{CVaR}$ & 0.1         & 0.13                                    &7\%                                           \\[1.5pt]
\midrule
$\mathrm{EVaR}$ & 0.8            & 0.10                                  &13\%                                            \\[1.5pt]
$\mathrm{EVaR}$ & 0.5          & 0.09                                 &4\%                                      \\[1.5pt]
$\mathrm{EVaR}$ & 0.1            & 0.09                                    &1\%                                       \\[1.5pt]
\midrule
\end{tabular}
\caption{Comparison between conditional expectation, CVaR, and EVaR coherent risk measures in 100 Monte Carlo simulations.  }
\end{table}

For the sake of illustration, Figure~\ref{fig:mdp} shows the trajectories of system~\eqref{eq:dcpcvrrrar} with risk-neutral, CVaR, and EVaR controllers ($\beta=0.8$) with initial conditions $(-1,1)$.

      \begin{figure*}[!h] \centering{
%\includegraphics[scale=.3]{mdpexample.png}\\
\includegraphics[scale=.29]{Figures/meanreach.eps}~
\hspace{.12cm}
\includegraphics[scale=.29]{Figures/cvarreach.eps}
\hspace{.12cm}
\includegraphics[scale=.29]{Figures/evarreach.eps}
\vspace{-0cm}
\caption{Risk-sensitive finite-time reachability enforcement results for the Example I with total expectation (left), CVaR (middle), and EVaR (right) coherent risk measures for 50 Monte Carlo simulations. The dashed lines show the boundaries of $h_i$, $i=1,2,3,4$. The goal region is the square intersection of $h_i$, $i=1,2,3,4$.}\label{fig:mderre3p}
%\vspace{-0.5cm}
} 
 \end{figure*}
 
       \begin{figure}[!h] \centering{
%\includegraphics[scale=.3]{mdpexample.png}\\
\includegraphics[scale=.31]{Figures/evarreachinput.eps}~
\caption{Evolution of the control signals for the risk-sensitive EVaR controller with $\beta=0.2$ in $50$ Monte Carlo experiments. }\label{fig:mderereerre3p}
%\vspace{-0.5cm}
} 
 \end{figure}

\subsubsection{$\rho$-reachability}:  We considered an square, goal region, which is defined as the intersection of the following hyperspaces
\begin{equation*}
    \begin{cases}
    h_1(x) = x_1 +2 > 0,\\
    h_2(x) = -x_1 +2 > 0,\\
    h_3(x) = x_2 +2 > 0,\\
        h_4(x) = -x_2 +2 > 0.\\
    \end{cases}
\end{equation*}
Hence, the goal set can be defined as
$$
\mathcal{S} = \left \{ x \in \mathbb{R}^2 \mid \land_{i=1}^4 (h_i(x) > 0) \right \}.
$$
From Proposition 2, we infer that it suffices to choose $h(x) = \min \{h_1(x),h_2(x),h_3(x),h_4(x)\}$. Similar to previous section,   the control bounds were chosen as $u \in [-5,5]$. 

 

Figure~\ref{fig:mderre3p} depicts the obtained results for risk-neutral, CVaR, EVaR controllers with $\beta=0.2$ and initial condition $(4,0)$ in 50 Monte Carlo experiments. As it can be seen from the figures all controllers achieve finite-time reachability. However, in the risk-neutral case, after the trajectories reach the goal region, they violate the safety requirement in multiple occasions (11 out of 50 runs). CVaR-based controller fares better with less (4 out of 50) violations and EVaR-based controller incurs no violations. 

The set of parameters selected for the risk-neutral, CVaR, and EVaR controllers were preset respectively as
$$
\begin{cases}
\gamma = 0.9 \\
\varepsilon = 16.2,
\end{cases}
~~
\begin{cases}
\gamma = 0.9\\
\varepsilon = 6.5,
\end{cases}
\text{and}~~\begin{cases}
\gamma = 0.9 \\
\varepsilon = 4 .
\end{cases}
$$
Given that $\min \{h_1(x_0),h_2(x_0),h_3(x_0),h_4(x_0)\} = -2$, from~\eqref{eq:disjtbBF1time} in Proposition 2, we obtain  $t^* \le 1.1$, $t^* \le 2.5$, and $t^* \le 3.8$ for risk-neutral, CVaR, and EVaR controllers, respectively. This is also consistent with the Monte Carlo simulations depicted in Figure~\ref{fig:mderre3p}. In fact, as the controller becomes more risk-sensitive (for example, CVaR versus EVaR), it may take longer for the system to reach the goal region but in return there is a higher guarantee of safety once inside this~set.


The risk-sensitive EVaR control signals are also provided in Figure~\ref{fig:mderereerre3p}. Note that the control signals respect the input bounds.

  
%   \subsection{Example II: Application to Underactuated Bipedal Walking}
%   \input{walkingExample}

==> Sections/synthesis.tex <==
\section{Enforcing Risk Control Barriers}

In this section, we show how RCBFs can be implemented to guarantee safety of nonlinear discrete-time dynamical systems. We begin with the general, nonlinear optimization problem.

\textbf{RCBF Primal Optimization:} At every time step $t$, given $x^t$, a set $\mathcal{S}$ as described in~\eqref{eq:safeset}, the coherent risk measure $\rho$, control upper bounds $\overline{u}$ and lower bounds $\underline{u}$, the convex function $\alpha \in \mathcal{K}$ (satisfying $\alpha(r) < r$ for all $r>0$) or constants $\varepsilon>0$ and $\gamma \in (0,1)$, solve 
\begin{subequations} \label{eq:mainopt}
\begin{align}
    u^t_* = &\argmin_{u^t}~~ (u^t)^T u^t \nonumber \\
            &\text{subject to} \nonumber \\
            & \quad  \underline{u} \le u^t \le \overline{u}, \label{eq:controlbounds} \\
             & \quad   \rho \left( h(f(x^t,u^t,w)\right) \ge  \alpha( h(x^{t})), \label{eq:conssafe}  \\
             &\text{or} \nonumber \\
            &    \quad \rho\left({h}(f(x^t,u^t,w))\right)-\gamma {h}(x^{t}) \ge \varepsilon (1-\gamma), \label{eq:consreach}
\end{align}
\end{subequations}
where the choice of constraint~\eqref{eq:conssafe} or~ constraint \eqref{eq:consreach} depends on which property we are interested in enforcing. Note that instantaneous controls $u^t$ are the only variables in the optimization.

For general nonlinear $h$, optimization problem~\eqref{eq:mainopt} is a nonlinear program in the decision variable $u^t$ ($\rho$ is a convex function in $h$). Indeed, this was the case for optimization problems designed for enforcing discrete control barrier functions for discrete-time systems even without stochastic uncertainty~\cite{agrawal2017discrete}. In this setting, MATLAB functions such as \texttt{fmincon} can be used to solve the nonlinear program. 

\textbf{RCBF Dual Optimization:} Note that for any coherent risk measure, an equivalent nonlinear optimization problem can be written using its dual.

\begin{subequations} \label{eq:dual_rcbf}
\begin{align}
    u^t_* = &\argmin_{u^t}~~ (u^t)^T u^t \nonumber \\
            &\text{subject to} \nonumber \\
            & \quad  \underline{u} \le u^t \le \overline{u}, \label{eq:controlbounds} \\
            & \quad  \forall p \in \mathcal{P}, \nonumber \\
             & \quad   \mathbb{E}_p \left[ h(f(x^t,u^t,w)\right] \ge  \alpha( h(x^{t})), \label{eq:conssafe}  \\
             &\text{or} \nonumber \\
            & \quad \mathbb{E}_p \left[{h}(f(x^t,u^t,w))\right]-\gamma {h}(x^{t}) \ge \varepsilon (1-\gamma). \label{eq:consreach}
\end{align}
\end{subequations}

In the following subsections, we will show how these nonlinear optimization problem can be solved efficiently, depending on the structure of the system.

\subsection{DCPs for Convex RCBFs}

Here, we restrict our attention to the case when system~\eqref{eq:dynamics} is a control-affine system. That is, $$x^{t+1}=f(x^t,w^t)+g(x^t,w^t)u^t,$$ where $f: \mathcal{X} \times \mathcal{W} \to \mathbb{R}^{n}$ and $g: \mathcal{X} \times \mathcal{W} \to \mathbb{R}^{n \times m}$. Here, the disturbance $w^t$ can enter the system in any way.

To guarantee convexity of the resulting optimization problem, we assume that the RCBF is convex. 
Then, the term~$\rho\left({h}(x^{t+1})\right)$ in constraints ~\eqref{eq:conssafe} and \eqref{eq:consreach} changes to 
$$
\rho\left(h(f(x^t,w^t)) + h(g(x^t,w^t) u^t)\right).
$$

It is important to note that this equation is convex in $u^t$ \cite{boyd2004convex}(Equation 3.10), as $h(\cdot)$ is convex in $x^{t+1}$ (and thus $u^t$), and $\rho(\cdot)$ is convex and non-decreasing, since it is a coherent risk measure. 

Re-writing optimization problem~\eqref{eq:mainopt}, letting $\alpha \in (0,1)$ be a constant, gives the following optimization problem

\begin{subequations} \label{eq:mainoptlinear}
\begin{align}
    u^t_* & = \argmin_{u^t}~~ (u^t)^T u^t \nonumber \\
            &\text{subject to} \nonumber \\
            & \quad  \underline{u} \le u^t \le \overline{u}, \label{eq:controlboundsL} \\
             & \quad   \rho\left(h(f(x^t,w^t)) + h(g(x^t,w^t) u^t)\right) \ge  \alpha \left( h(x^t) \right), \label{eq:conssafeL}  \\
             &\text{or} \nonumber \\
            &    \quad  \rho\left(h(f(x^t,w^t)) + h(g(x^t,w^t) u^t)\right)-\gamma \left( h(x^t) \right) \nonumber \\ & \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad   \ge \varepsilon (1-\gamma). \label{eq:consreachL}
\end{align}
\end{subequations}

Optimization~\eqref{eq:mainoptlinear} is a difference convex program. In fact, we can write~\eqref{eq:mainoptlinear} in a standard DCP form as follows
\begin{subequations}\label{eq:DCP}
\begin{align}
     u^t_* = & \argmin_{u^t}~~ q_0(u^t)  \nonumber  \\
        &\text{subject to} \nonumber  \\
        & \quad q_1(u^t) \le 0~\text{and}~q_2(u^t) \le 0,  \\
        & \quad q_3 - q_4(u^t) \le 0, \\
        &\text{or} \nonumber  \\
        &\quad  q_5 -  q_4(u^t) \le 0, 
\end{align}
\end{subequations}
wherein $q_0(u^t) = (u^t)^T u^t$ is a convex (quadratic) function, $q_1(u^t)=\underline{u}-u^t$ is a convex (linear) function, $q_2(u^t)=u^t - \overline{u}$ is a convex (linear) function, $q_3=\alpha \left( h(x^t) \right)$ is a convex (constant) function,  \begin{equation*}q_4=\rho\left(h(f(x^t,w^t)) + h(g(x^t,w^t) u^t)\right)\end{equation*} is a convex function in $u^t$ since $\rho$ is a coherent risk measure, and $q_5= \gamma \left(h(x^t) \right)+\varepsilon (1-\gamma)$ is a convex (constant) function.

 DCPs like ~\eqref{eq:DCP} arise in  many applications, such as feature selection in  machine learning~\cite{le2008dc} and inverse covariance estimation in statistics~\cite{thai2014inverse}. Although DCPs can be solved globally~\cite{horst1999dc}, \textit{e.g.} using branch and bound algorithms~\cite{lawler1966branch}, a locally optimal solution can be obtained based on techniques of nonlinear optimization~\cite{Bertsekas99} more efficiently. In particular, in this work, we use a variant of the convex-concave procedure~\cite{lipp2016variations,shen2016disciplined}, wherein  the concave terms are replaced by a convex upper bound and solved. In fact, the disciplined convex-concave programming (DCCP)~\cite{shen2016disciplined} technique linearizes DCP problems into a (disciplined) convex program (carried out automatically via the DCCP  package~\cite{shen2016disciplined}), which is then converted into an equivalent cone program by
replacing each function with its graph implementation. Then, the cone program can be solved readily by available convex programming solvers, such as CVX~\cite{cvx}. 

At this point, we should point out that solving~\eqref{eq:DCP} via the 
DCCP method, finds the (local) saddle points to optimization problem ~\eqref{eq:DCP}. However, every such local $u^t$ guarantees $\rho$-safety or $\rho$-reachability.

\textbf{Example:} Consider a (continuous-time, nonlinear) cart-pole system with states $X = \left[x, \theta \right] ^T$:
\begin{equation*}
    \dot{X} = 
    \begin{bmatrix}
    \dot{x} \\
    \dot{\theta} \\
    \frac{1}{m_c + m_p \sin^2\theta}\left[ u + m_p \sin\theta (l \dot\theta^2 + g\cos\theta)\right] \\
    \frac{1}{l(m_c + m_p \sin^2\theta)} \left[ -u
       \cos\theta - m_p l \dot\theta^2 \cos\theta \sin\theta - (m_c + m_p) g \sin\theta \right] + w
    \end{bmatrix}
\end{equation*}

Here, the disturbance $w \in \mathcal{W}$ enters the system through $\ddot{\theta}$. The set of disturbances is chosen to be 
$$
\mathcal{W} = \{-.2, -.1, 0, .1, .2 \},
$$
with the probabilities of each being equality distributed (0.2).

The discrete-time dynamics are chosen to be an Euler integration of the continuous-time dynamics, with a time-step of 0.1 seconds.

Now, consider the barrier function
\begin{equation*}
    h(x) = (\theta - \theta_0)^2 - C = \theta^2 - \theta \theta_0 + \theta_0^2 - C.
\end{equation*}

The coherent risk measure chosen is EVaR, with a value of $\beta = .25$.

Utilizing \eqref{eq:mainoptlinear}, we enforce the RCBF over 100 simulations with randomly chosen disturbances.

\subsection{Convex Programs for Dual RCBFs}

In this section, we look at the dual RCBF formulation to produce convex programs. This comes at the cost of generality in how the uncertainty enters the system, but results in faster solving problems with guarantees of optimality.

The dual RCBF formulation \eqref{eq:dual_rcbf} features a robust constraint in the variable $w$, which lies in some uncertainty region defined by the coherent risk measure. To make this problem tractable, we must find the robust counterpart of this robust constraint. This process is demonstrated over a wide variety of uncertainty regions in \cite{ben2015deriving}, which we will utilize for the remainder of this section. 

Suppose we have the constraint
% \begin{equation}
%     \min_{w \in \mathcal{W}} h(w,x) \geq 0,
%     \label{eq:robust_opt}
% \end{equation}
\begin{equation}
    \max_{w \in \mathcal{W}} f(w,x) \leq 0,
    \label{eq:robust_opt}
\end{equation}
where $x \in \mathbb{R}^n$ is the optimization variable and $w \in \mathbb{R}^m$ is the uncertain variable. We define the uncertainty set as
\begin{equation}
    \mathcal{W} = \left\{ w = w^0 + Az | z \in Z \subset \mathbb{R}^L \right\}
\end{equation}
where $w^0 \in \mathbb{R}^m$ is the nominal value of uncertainty, $A \in \mathbb{R}^{(m \times L)}$, and Z is nonempty, convex, and compact. %We have that
% \begin{align}
%     &\min_{w \in \mathcal{W}} h(w,x) \\
%     =&\min_{w \in \mathbb{R}^m} \{h(w,x) + \delta(a,\mathcal{W})\}\\
%     =&\max_{w \in \mathbb{R}^m}
% \end{align}

From Fenchel duality, we have that if a pair $(x,v)$ satisfies the constraint
\begin{align}
    (w^0)^Tv + \delta ^*(A^Tv | Z) - f_*(v,x) \leq 0,
    \label{eq:frc}
\end{align}
then $x$ satisfies \eqref{eq:robust_opt}. Moreover, strong duality occurs if $f(w,x)$ is concave in $w$. Here, $\delta^*$ is the support function,
$$
\delta^*(y|S) = \sup_{x \in S}y^Tx,
$$
and $f_*$ is the partial concave conjugate of $f$,
$$
f_*(v,y) = \inf_{x \in \rm{dom}(f)}\{v^Tx-f(x,y)\}.
$$



It is important to note that if $f(w,x)$ is convex in $x$, then the constraint \eqref{eq:frc} is convex.

To obtain our constraint \eqref{eq:conssafeL} in the form of \eqref{eq:robust_opt}, we first reverse the sign
\begin{align}
    - \rho\left(h(g(x^t,w^t) u^t)\right) - \rho\left(h(f(x^t,w^t))\right) + \alpha \left( h(x^t) \right) \leq 0,
\end{align}
then we substitute the coherent risk measure in its dual form
\begin{align}
    - \max_{p \in \mathcal{P}}\mathbb{E}_p[h(p,u^t)] - \rho\left(h(f(x^t,w^t))\right) + \alpha \left( h(x^t) \right) \leq 0.
\end{align}
Here, we omit the dependence of $h$ on $x^t$ to highlight the decision variables $p$ and $u^t$. Finally, using Fenchel duality and setting the uncertainty set $\mathcal{W} = \mathcal{Z}$ ($w^0 = 0$, $A = I_{m\times m})$, we have
\begin{align}
    -\delta^*(v | \mathcal{P}) + \mathbb{E}_v[h(v,u^t)]_* - \rho\left(h(f(x^t,w^t))\right) + \alpha \left( h(x^t) \right) \leq 0.
\end{align}

Note that $\mathbb{E}_p[h(p,u^t)] = \underset{p_i \in \mathcal{P}}{\sum}p_ih(p_i,u^t)$. Now, using \cite{ben2015deriving}[Tables 1 and 2], the values of $h_*(v,u^t)$ and $\delta^*(v | \mathcal{P})$ can be found. In the following section, we illustrate how affine constraints result from a linear RCBF with linear uncertainty.

\subsection{Quadratic Programs for Linear RCBFs}

\vspace{0.2cm}
\begin{defn}[Polytopic Risk Measure]
    \textit{A \emph{polytopic risk measure} is a risk measure $\rho:\mathcal{H}_{t}\to \mathcal{H}_{t-1}$ with a dual representation:}
\begin{equation}
\rho(h) = \max_{p \in \mathcal{P}}\mathbb{E}_p[h],
\end{equation}
\textit{such that the risk envelope $\mathcal{P}$ is polytopic.}
\end{defn}
\vspace{0.2cm}

An example of one such risk measure is CVaR, whose polytopic risk envelope is given by 

\begin{equation}
    \mathcal{P} = \left\{ q \in \Delta^M \ | \ 0 \leq q(j) \leq \frac{p(j)}{\alpha},\  j \in \{ 1,...,M\} \right\}.
\end{equation}

Now, without loss of generality, assume the polytopic risk measure is given by the polytope $\mathcal{P} = \{c | Bc \leq b \}$. Now, we have
\begin{align}
    \delta^*(v | \mathcal{P}) &=  \max_{c}\{ v^Tc \ | \  Bc \leq b\} \\
    &= \min_{d}\{ b^T d\  |\  B^Td = v,\ d \geq 0\}
\end{align}
Thus, we can rewrite the constraint as 
\begin{align*}
    &-b^T d + \mathbb{E}_v[h(v,u^t)]_* - \rho\left(h(f(x^t,w^t))\right) + \alpha \left( h(x^t) \right) \leq 0, \\
    &B^T d = v, \\
    &d \geq 0.
\end{align*}.

Now that $\delta^*(v|\mathcal{P})$ is given as a sequence of affine constraints, we simply need an affine expression for $\mathbb{E}_v[h]_*(v,u^t)$. Assume that $h(x)$ takes the form
\begin{align}
    h(x) = Hx + l,
\end{align}
and assume that the uncertain term $w$ enters linearly,
\begin{align}
    h(w,x) = w^Th(x) = w^THx + w^Tl
\end{align}
In this case, 
\begin{align}
    h_*(v,x) &= \inf_{a \in \mathbb{R}^m}\{a^Tv-a^Th(x,y)\}, \\
    &= 
    \begin{cases}
    0 & v = h(x)\\
    - \infty & v \neq h(x)
    \end{cases}.
\end{align}
With the addition of the $\mathbb{E}[]$ operator, the expression remains the same.

Therefore, the constraint becomes
\begin{align*}
    &-b^T d - \rho\left(h(f(x^t,w^t))\right) + \alpha \left( h(x^t) \right) \leq 0, \\
    &B^T d = Hf(x^T) + Hg(x^T)u^T + l , \\
    &d \geq 0.
\end{align*}.

This constraint is affine in the decision variables $d$ and $u^T$, making the RCBF easily enforced in real-time.

==> Sections/synthesis_old.tex <==
\section{Risk Control Barrier Function Synthesis}

Inspired by the quadratic programming formulations of conventional control barrier functions in the continuous-time case~\cite{ames2016control}, we pose the controller synthesis problem as an optimization.

\textbf{RCBP Synthesis Optimization:} At every time step $t$, given $x^t$, a set $\mathcal{S}$ as described in~\eqref{eq:safeset}, the coherent risk measure $\rho$, control upper bounds $\overline{u}$ and lower bounds $\underline{u}$, the convex function $\alpha \in \mathcal{K}$ (satisfying $\alpha(r) < r$ for all $r>0$) or constants $\varepsilon>0$ and $\gamma \in (0,1)$, solve 
\begin{subequations} \label{eq:mainopt}
\begin{align}
    u^t_* = &\argmin_{u^t}~~ (u^t)^T u^t \nonumber \\
            &\text{subject to} \nonumber \\
            & \quad  \underline{u} \le u^t \le \overline{u}, \label{eq:controlbounds} \\
             & \quad   \rho \left( h(f(x^t,u^t,w)\right) \ge  \alpha( h(x^{t})), \label{eq:conssafe}  \\
             &\text{or} \nonumber \\
            &    \quad \rho\left({h}(f(x^t,u^t,w))\right)-\gamma {h}(x^{t}) \ge \varepsilon (1-\gamma), \label{eq:consreach}
\end{align}
\end{subequations}
 where the choice of constraint~\eqref{eq:conssafe} or~ constraint \eqref{eq:consreach} depends on which property we are interested in enforcing. Note that instantaneous controls $u^t$ are the only variables in the optimization.

For general nonlinear $h$, optimization problem~\eqref{eq:mainopt} is a nonlinear program in the decision variable $u^t$ ($\rho$ is a convex function in $h$). Indeed, this was the case for optimization problems designed for synthesizing discrete control barrier functions for discrete-time systems even without stochastic uncertainty~\cite{agrawal2017discrete}. In this setting, MATLAB functions such as \texttt{fmincon} can be used to solve the nonlinear program. 

Next, we show that, for linear discrete-time systems with stochastic uncertainty, we can compute RCBFs via difference convex programs. 

\subsection{DCPs for RCBF Synthesis for Linear Systems}

For the remainder of this section, we restrict our attention to the case when system~\eqref{eq:dynamics} is a linear system. That is, $$f(x^t,u^t,w^t)=A(w^t)x^t+B(w^t)u^t+G(w^t),$$ where $A: \mathcal{W} \to \mathbb{R}^{n \times n}$, $B: \mathcal{W} \to \mathbb{R}^{n \times m}$ and $G: \mathcal{W} \to \mathbb{R}^{n}$.

For such systems, we assume the RCBF takes the form of a linear function
\begin{equation}\label{eq:RCBFlinear}
    h(x^t) = H x^t + l,
\end{equation}
where $H \in \mathbb{R}^{1\times n}$ and $l \in \mathbb{R}$. 
Then, the term~$\rho\left({h}(f(x^t,u^t,w)\right)$ in constraints ~\eqref{eq:conssafe} and \eqref{eq:consreach} changes to 
$$
\rho(H A(w)x^t+H B(w) u^t +HG(w) +l).
$$
Hence, $\rho$ becomes a convex function in $u^t$ the control variable. 

Re-writing optimization problem~\eqref{eq:mainopt} for linear discrete time systems with stochastic uncertainty, letting $\alpha \in (0,1)$ be a constant, and RCBF~\eqref{eq:RCBFlinear} gives  the following optimization problem

\begin{subequations} \label{eq:mainoptlinear}
\begin{align}
    u^t_* & = \argmin_{u^t}~~ (u^t)^T u^t \nonumber \\
            &\text{subject to} \nonumber \\
            & \quad  \underline{u} \le u^t \le \overline{u}, \label{eq:controlboundsL} \\
             & \quad   \rho\left(H A(w)x^t+H B(w) u^t +HG(w) +l\right) \ge  \alpha H x^t +\alpha l, \label{eq:conssafeL}  \\
             &\text{or} \nonumber \\
            &    \quad  \rho\left(H A(w)x^t+H B(w) u^t +HG(w) +l\right)-\gamma H x^t -\gamma l \nonumber \\ & \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad   \ge \varepsilon (1-\gamma). \label{eq:consreachL}
\end{align}
\end{subequations}

Optimization~\eqref{eq:mainoptlinear} is a difference convex program. In fact, we can write~\eqref{eq:mainoptlinear} in a standard DCP form as follows
\begin{subequations}\label{eq:DCP}
\begin{align}
     u^t_* = & \argmin_{u^t}~~ q_0(u^t)  \nonumber  \\
        &\text{subject to} \nonumber  \\
        & \quad q_1(u^t) \le 0~\text{and}~q_2(u^t) \le 0,  \\
        & \quad q_3 - q_4(u^t) \le 0, \\
        &\text{or} \nonumber  \\
        &\quad  q_5 -  q_4(u^t) \le 0, 
\end{align}
\end{subequations}
wherein $q_0(u^t) = (u^t)^T u^t$ is a convex (quadratic) function, $q_1(u^t)=\underline{u}-u^t$ is a convex (linear) function, $q_2(u^t)=u^t - \overline{u}$ is a convex (linear) function, $q_3=\alpha H x^t +\alpha l$ is a convex (constant) function,  \begin{equation*}q_4=\rho\left(H A(w)x^t+H B(w) u^t +HG(w) +l\right)\end{equation*} is a convex function in $u^t$ since $\rho$ is a coherent risk measure, and $q_5= \gamma H x^t + \gamma l+\varepsilon (1-\gamma)$ is a convex (constant) function.

 DCPs like ~\eqref{eq:DCP} arise in  many applications, such as feature selection in  machine learning~\cite{le2008dc} and inverse covariance estimation in statistics~\cite{thai2014inverse}. Although DCPs can be solved globally~\cite{horst1999dc}, \textit{e.g.} using branch and bound algorithms~\cite{lawler1966branch}, a locally optimal solution can be obtained based on techniques of nonlinear optimization~\cite{Bertsekas99} more efficiently. In particular, in this work, we use a variant of the convex-concave procedure~\cite{lipp2016variations,shen2016disciplined}, wherein  the concave terms are replaced by a convex upper bound and solved. In fact, the disciplined convex-concave programming (DCCP)~\cite{shen2016disciplined} technique linearizes DCP problems into a (disciplined) convex program (carried out automatically via the DCCP  package~\cite{shen2016disciplined}), which is then converted into an equivalent cone program by
replacing each function with its graph implementation. Then, the cone program can be solved readily by available convex programming solvers, such as CVX~\cite{cvx}. 

At this point, we should point out that solving~\eqref{eq:DCP} via the 
DCCP method, finds the (local) saddle points to optimization problem ~\eqref{eq:DCP}. However, every such local $u^t$ guarantees $\rho$-safety or $\rho$-reachability.

\subsection{DCPs for Conditional Expectation, CVaR, and EVaR} \label{sec:DCPcomput}

In this section, we present DCP~\eqref{eq:DCP} for conditional total expectation, CVaR, and EVaR coherent risk measures defined in Section~\ref{sec:riskexamples}, which are used in our numerical experiments. 

For total conditional expectation, DCP~\eqref{eq:DCP} changes to a quadratic program. In fact, the coherent risk term $q_4=\rho\left(H A(w)x^t+H B(w) u^t +HG(w) +l\right)$  simplifies to  
\begin{equation}\label{cscseee}
\sum_{i=1}^{|\mathcal{W}|}  \left(H A(w_i)x^t+H B(w_i) u^t +HG(w) +l\right)p(w_i), 
\end{equation}
which is linear in the decision variable $u^t$. Hence, DCP~\eqref{eq:DCP} has a quadratic objective subject to linear constraints, which is a quadratic program.



For CVaR, the coherent risk term $q_4=\rho\left(H A(w)x^t+H B(w) u^t +HG(w) +l\right)$  simplifies to  
\begin{multline}\label{cscseee}
\inf_{\zeta \in \mathbb{R}} \bigg\{ \zeta +\frac{1}{\beta} \sum_{i=1}^{|\mathcal{W}|}  \big(H A(w_i)x^t+H B(w_i) u^t \\+ HG(w_i)  +l -\zeta\big)_{+}p(w_i)       \bigg\}, 
\end{multline}
which has the extra decision variable $\zeta \in \mathbb{R}$. Hence, DCP~\eqref{eq:DCP} can be rewritten as 
\begin{subequations}\label{eq:DCPcvar}
\begin{align}
     u^t_* = & \argmin_{u^t,\zeta}~~ q_0(u^t)  \nonumber  \\
        &\text{subject to} \nonumber  \\
        & \quad q_1(u^t) \le 0~\text{and}~q_2(u^t) \le 0,  \\
        & \quad q_3 - \hat{q_4}(\zeta,u^t) \le 0, \\
        &\text{or} \nonumber  \\
        &\quad  q_5 -  \hat{q_4}(\zeta,u^t) \le 0, 
\end{align}
\end{subequations}
where the expression for $\hat{q_4}(\zeta,u^t)$ is given in~\eqref{cscseee}. Note that $\hat{q_4}(\zeta,u^t)$ above is  convex in $\zeta$~\cite[Theorem 1]{rockafellar2000optimization} because the function $(\cdot)_+$ is increasing and convex~\cite[Lemma A.1., p. 117]{ott2010markov}.



% In fact, Theorem 1 can applied to CVaR since it is a coherent risk measure. For an MDP $\mathcal{M}$, the risk value functions can be computed by DCP~\eqref{eq:DCP}, where 
% $$
% g_2({V}_\gamma) = \inf_{\zeta\in \mathbb{R}} \left\{ \zeta + \frac{1}{\varepsilon} \sum_{s' \in \mathcal{S}}\left(V_\gamma(s')-\zeta\right)_{+} T(s'\mid s,\alpha)        \right\},
% $$
% where the infimum on the right hand side of the above equation can be absorbed into the overal infimum problem, \textit{i.e.,} $\inf_{\boldsymbol{V}_\gamma,\boldsymbol{\lambda} \succeq \boldsymbol{0},\zeta}$. 




For $\mathrm{EVaR}_\beta$, the coherent risk term $q_4=\rho\left(H A(w)x^t+H B(w) u^t +l\right)$  simplifies to  
\begin{multline}\label{cscseeevar}
\inf_{\zeta >0} \bigg\{ \frac{1}{\zeta} \log\Big(\frac{1}{\beta} \sum_{i=1}^{|\mathcal{W}|}  e^{\zeta \left(H A(w_i)x^t+H B(w_i) u^t +HG(w_i) +l\right) } \\ \times p(w_i) \Big)        \bigg\}, 
\end{multline}
which has the extra decision variable $\zeta >0$. Since $\zeta>0$, using the change of variables, $\hat{u}^t=\zeta u^t$ (note that this change of variables is monotone increasing in $\zeta$~\cite{agrawal2018rewriting}), DCP~\eqref{eq:DCP} can be converted to 
\begin{subequations}\label{eq:DCPevar}
\begin{align}
     \hat{u}^t_* = & \argmin_{{\hat{u}}^t,\zeta>0}~~ q_0(\hat{u}^t)  \nonumber  \\
        &\text{subject to} \nonumber  \\
        & \quad \hat{q_1}(\hat{u}^t,\zeta) \le 0~\text{and}~\hat{q_2}(\hat{u}^t,\zeta) \le 0,  \\
        & \quad \hat{q_3}(\zeta) - \tilde{q_4}(\zeta,\hat{u}^t) \le 0, \\
        &\text{or} \nonumber  \\
        &\quad  \hat{q}_5(\zeta) -  \tilde{q_4}(\zeta,\hat{u}^t) \le 0, 
\end{align}
\end{subequations}
where $\hat{q_1}(\hat{u}^t,\zeta)=\zeta\underline{u}-\hat{u}^t$, $\hat{q_1}(\hat{u}^t,\zeta)=\hat{u}^t -\zeta\overline{u}$, $\hat{q_3}(\zeta)=\zeta q_3$, $\hat{q_5}(\zeta)=\zeta q_5$, and 
\begin{equation}
\tilde{q_4}(\zeta,\hat{u}^t) = \scriptstyle  \log\left(\frac{1}{\beta} \sum_{i=1}^{|\mathcal{W}|}  e^{ \left(\zeta H A(w_i)x^t+H B(w_i)\hat{u}^t +\zeta HG(w_i)  +\zeta l \right) }p(w_i) \right). \nonumber
\end{equation}
 
  Note that $\tilde{q_4}(\zeta,\hat{u}^t) $ is  convex in  $\hat{u}^t$, since the logarithm of sums of exponentials is convex~\cite[p.~72]{boyd2004convex}. 
  
  We end this section by making a remark for Markov polytopic risk measure such as the ones studied in~\cite{chow2014framework}. Markov polytopic risk measures can be represented as
  \begin{equation} \label{cs3cwd}
  \rho(Z) = \max_{\psi \in \mathcal{Q}} \mathbb{E}_\psi( Z),
  \end{equation}
  where $\psi$ is a probability density function belonging to a  polytopic set $\mathcal{Q}$ ($\mathcal{Q}$ is a convex set for general coherent risk measures~\cite[Theorem 6.6]{shapiro2014lectures}). 
%   Then, DCP~\eqref{eq:DCP} turns into a quadratic program. This is simply because, for system~\eqref{eq:dynamics}, $\mathbb{E}_\psi(Z) = \sum_{i=1}^{|\mathcal{W}|} Z(w_i)\psi(w_i) $ and $\psi \in \mathcal{Q}$ is a linear constraint since $\mathcal{Q}$ is a polytope.
  However, despite the fact that many coherent risk measures can be described by~\eqref{cs3cwd} with $\mathcal{Q}$ being a polytope, such as CVaR, this is not the case in general. For example, for the EVaR risk measure, the set $\mathcal{Q}$ takes the form of an exponential cone~\cite{kocuk2020conic,Anushri2020}. DCP formulation in this section is more general in that it provides a unified computational framework for any coherent risk measure.
